DeepSDF: Learning Continuous Signed Distance Functions for Shape Representation

Computer graphics, 3D computer vision and robotics communities have produced multiple approaches to representing 3D geometry for rendering and reconstruction. These provide trade-offs across fidelity, efficiency and compression capabilities. In this work, we introduce DeepSDF, a learned continuous Signed Distance Function (SDF) representation of a class of shapes that enables high quality shape representation, interpolation and completion from partial and noisy 3D input data. DeepSDF, like its classical counterpart, represents a shape's surface by a continuous volumetric field: the magnitude of a point in the field represents the distance to the surface boundary and the sign indicates whether the region is inside (-) or outside (+) of the shape, hence our representation implicitly encodes a shape's boundary as the zero-level-set of the learned function while explicitly representing the classification of space as being part of the shapes interior or not. While classical SDF's both in analytical or discretized voxel form typically represent the surface of a single shape, DeepSDF can represent an entire class of shapes. Furthermore, we show state-of-the-art performance for learned 3D shape representation and completion while reducing the model size by an order of magnitude compared with previous work.

==> mktex <==
#!/usr/bin/env python

import os, re, time, argparse
import subprocess as sub

def pdfCompile(haveBib,main):
  print 'compiling {}'.format(main)
  if sub.call(['pdflatex',main]) > 0:
    return
  if haveBib:
    if sub.call(['bibtex',re.sub('tex','aux',main)]) > 0:
      return
    sub.call(['pdflatex',main])
  sub.call(['pdflatex',main])

parser = argparse.ArgumentParser(description = 'make tex file')
parser.add_argument('-c','--continuous', action='store_true',                   
    help='keeps cheching of files have changed and recompiles if so')
parser.add_argument('-r','--recompile', action='store_true',                   
    help='recompile from scratch')
parser.add_argument('-i','--input', help='file name of specific file'\
    +' to compile. If not specified all main fails will be compiled')
args = parser.parse_args()                                                      

texFiles = []
#for subdir, dirs, files in os.walk('./'):
for f in os.listdir('./'):
  if os.path.splitext(f)[1] in ['.tex','.bib']:
    print f
    texFiles.append(f)

print ' ------- making ----------'
mainTexs = ['main.tex','writeup.tex','poster.tex']

mains = []
haveBib = False
if not args.input is None:
  print 'using input {} as as main tex file for compilation'.format(args.input)
  mains = [args.input]
  # try finding a bib file
  for f in texFiles:
    if os.path.splitext(f)[1] == '.bib' and os.path.split(f)[0] == '':
      haveBib = True
      print 'found bibtex file {}'.format(f)
else:
  print 'no input main given => finding it in the current folder'
  # try finding the main by common names I give them
  for f in texFiles:
    print os.path.splitext(f), os.path.split(f)
    if os.path.split(f)[1] in mainTexs and os.path.split(f)[0] == '':
      mains = [f]
      print 'found main tex file {}'.format(f)
    elif os.path.splitext(f)[1] == '.bib' and os.path.split(f)[0] == '':
      haveBib = True
      print 'found bibtex file {}'.format(f)
  # now try finding the main by looking for a \begin{document} in the files
  if len(mains) == 0:
    print 'looking for mains using \\begin\{document\}'
    for f in texFiles:
      print 'searching in {}'.format(f)
      for line in open(f):
        #print line[:-1]
        if not re.search('begin{document}',line) is None:
          mains.append(f)
          print ' found \begin{document}'+' in {} -> adding as main file'.format(f)
          break

if mains[0] is None or len(mains) == 0 :
  print "no main found {}".format(mainTexs)
else:
  if args.continuous:
    lastT = [time.time() for f in texFiles]
    while 42:
      hasModification = False
      for j,f in enumerate(texFiles):
        modtime = os.stat(f).st_mtime
        #print '{} vs {}'.format(modtime,lastT[j])
        if modtime > lastT[j]:
          lastT[j] = modtime
          hasModification = True
          print '{} modified'.format(f)
      if hasModification:
        for main in mains:
          pdfCompile(haveBib,main)
      print 'sleeping'
      time.sleep(2)
  elif args.recompile:
    for main in mains:
      sub.call(['rm',re.sub('tex','aux',main)])
      pdfCompile(haveBib,main)
  else:
    for main in mains:
      print 'compile {}'.format(main)
      pdfCompile(haveBib,main)


==> tableUnknownCompletion.tex <==
 \begin{table}[t]
\centering
\footnotesize
 \begin{tabular}{|l|c|c|c|c|c|}
 \hhline{|=|=|=|=|=|=|}
  \multicolumn{1}{|l|}{\% compl., mean} & \multicolumn{1}{c|}{chair} & \multicolumn{1}{c|}{plane} & \multicolumn{1}{c|}{table} & \multicolumn{1}{c|}{lamp} & \multicolumn{1}{c|}{sofa}  \\
% \multicolumn{1}{cl|}{Method \& metric} & chair & plane & table & sofa & lamp & avg & inference\\
 \hline
 AtlasNet-Sph.  & 0.668 & 0.862 & 0.755 & 0.281 & 0.641  \\
 AtlasNet-25      & 0.723 & 0.887 & 0.785 & 0.528 & 0.681  \\
 DeepSDF        & \bf{0.947} & \bf{0.943} & \bf{0.959} & \bf{0.877} & \bf{0.931}  \\
 \hline
   \hhline{|=|=|=|=|=|=|}
%  CD, median    &    &  &   &   & \\
  \multicolumn{1}{|l}{\% compl., median} &  \multicolumn{1}{c}{ \ } &  \multicolumn{1}{c}{ \ } &  \multicolumn{1}{c}{ \ } &  \multicolumn{1}{c}{ \ }  &  \multicolumn{1}{c|}{} \\
 \hline
  AtlasNet-Sph.  & 0.686 & 0.930 & 0.795 & 0.257 & 0.666  \\
 AtlasNet-25      & 0.736 & 0.944 & 0.825 & 0.533 & 0.702  \\
 DeepSDF        & \bf{0.97} & \bf{0.970} & \bf{0.982} & \bf{0.930} & \bf{0.941}  \\
 \hline
  \hhline{|=|=|=|=|=|=|}
%  CD, median    &    &  &   &   & \\
  \multicolumn{1}{|l}{Cosine sim., mean} &  \multicolumn{1}{c}{ \ } &  \multicolumn{1}{c}{ \ } &  \multicolumn{1}{c}{ \ } &  \multicolumn{1}{c}{ \ }  &  \multicolumn{1}{c|}{} \\
 \hline
  AtlasNet-Sph.  & 0.790 & 0.840 & 0.826 & 0.719 & 0.847  \\
 AtlasNet-25      & 0.797 & 0.858 & 0.835 & 0.725 & 0.826  \\
 DeepSDF        & \bf{0.896} & \bf{0.907} & \bf{0.916} & \bf{0.862} & \bf{0.917}  \\
 \hline

   \end{tabular}
   \caption{Comparison of metrics  for representing unknown shapes (U) for various classes of ShapeNet. Mesh completion as defined in \cite{seitz2006comparison} i.e. the fraction of groundtruth sampled points that are within a $\delta$ (we used $\delta=0.01$) of the generated mesh, and mean cosine similarity is of normals for nearest groundtruth-generated point pairs.  Higher is better for all metrics in this table.} 
   \label{tab:4}
\end{table}

==> tablesOldUnused.tex <==

% \begin{table}[t]
% \centering
% \begin{tabular}{|l|r|r|l|}
% \hline

% Method                         & Fwd. pass         &  Inference & Inference \\
%  \textbackslash Metric. & time (s)  &  time (s)    & method  \\
%  \hhline{|=|=|=|=|}
%  \hline
% OGN                            &                          &    \multicolumn{1}{c|}{N/A}      & N/A \\
% \hline
% 3D-EPN                       &                       &                   &  Encoder   \\
% \hline
% AtlasNet-Sphere                      &                      &                   & Encoder\\
% \hline
% AtlasNet-25                      &                      &                   & Encoder \\
% \hline
% DeepSDF                    &                       & & Latent vector \\
%                                   &                         &  &optimization   \\
% \hline
% \end{tabular}
% \caption{Comparison of metrics for shape completion (C) from partial range scans of unknown chairs from ShapeNet. Metrics are described in detail in Appendix A.}
% \label{tab:chamfer}
% \end{table}


% \begin{table*}[t]
%   \centering
%   \begin{tabular}{|l|c|c|c|c|c|c|}
% \multicolumn{1}{l|}{}Method \& metric} & chair & plane & table & sofa & lamp & avg & inference\\
% \hhline{|=|=|=|=|=|=|=|}
% \hline
% AtlasNet-Sphere  & - & - & - & - & - & - \\
% AtlasNet-25      & - & - & - & - & - & - \\
% DeepSDF (ours)   & - & - & - & - & - & - \\
% \hline
%   \end{tabular}
%   \caption{Comparisons on lots of classes} %Some voxel/octree methods are occupancy-based, while \cite{dai2017shape} is a discrete voxel grid of SDF values.}
%   \label{tab:2}
% \end{table*}

% \begin{table}[t]
% \centering
% \begin{tabular}{|l|c|c|c|}
% \hline
% Method & Type & Res. & Topology\\
% \hline
% Vox-128 Oracle & Voxel (occ.) & 128^3 & - \\
% Vox-256 Oracle & Voxel (occ.) & 256^3 & - \\
% Vox-512 Oracle & Voxel (occ.) & 512^3 & - \\
% OGN \cite{ogn2017} & Octree (occ.) & 256^3 & - \\
% 3D-EPN \cite{dai2017shape} & Voxel (SDF) & 128^3 & $\mathcal{O}(128^3)$ \\
% AtlasNet \cite{groueix2018atlasnet} & Parametric mesh & \infty & 125 \\
% DeepSDF (ours) & Continuous SDF & \infty & \infty \\
% \hline
% \end{tabular}
% \caption{Overview of the benchmarked methods, including their shape representation type, resolution, and limits on number of topologically disconnected components. The voxel oracle methods \{Vox-256,Vox-512,Vox-1024\} measure the degradation alone due to voxelization (no learning). Some voxel/octree methods are occupancy-based, while \cite{dai2017shape} is a discrete voxel grid of SDF values. \js{I understand why we want to put $\infty$ into the table but I would argue that its not infinity - in both columns its something big but dependent on the number of parameters of the encoder. In fact this points to a whole nother research question of how does the parameter size and the expressiveness of the encoder relate? I would at least add a comment saying that its only theoretically infinite given enough model parameters. Infinite resolution is easier to defend than infinite topology}}
% \label{tab:methods}
% \end{table}

% \begin{table}[t]
% \centering
% \begin{tabular}{|l|c|c|c|c|}
% \hline
% Method & Memory (GB) & Time, inference (s)\\
% \hline
% OGN \cite{ogn2017} & 0.54 & 0.64 \\
% 3D-EPN \cite{dai2017shape} & 0 & 0  \\
% AtlasNet \cite{groueix2018atlasnet} & 0.172* & 5\\
% DeepSDF (ours) & 0.0074 & 7.5\\
% \hline
% \end{tabular}
% \caption{Performance comparison of the benchmarked learning methods.}% Not shown are the voxel oracle baselines, since they are not realistic methods.}
% \label{tab:performance}
% \end{table}




% \begin{table}[t]
% \centering
% \begin{tabular}{|l|c|c|c|c|c|}
% \hline
% Method \textbackslash Class & Chair & Table & Sofa & Plane & Car\\
% \hhline{|=|=|=|=|=|=|}
% Vox-128 Oracle & 0 & 0 & 0 & 0 & 0\\
% Vox-256 Oracle & 0 & 0 & 0 & 0 & 0\\
% Vox-512 Oracle &0 & 0 & 0 & 0 & 0\\
% \hline
% OGN \cite{ogn2017} &  - &  - & - & - & 0\\
% AtlasNet-S. \cite{groueix2018atlasnet}  & 1.81 & 1.88 & 1.73 & 0.98 & 1.75\\
% AtlasNet-25 \cite{groueix2018atlasnet}  & 1.56 & 1.52 & 1.83 & 0.87 & 1.58\\
% DeepSDF (ours)  & $\textbf{1.44}$ & 0 & 0 & $\textbf{0.77}$ & 0\\
% \hline
% \end{tabular}
% \caption{Reconstruction error of representing unseen shapes, measured by Chamfer Distance on models trained with an 80/20 split \cite{choy20163d} of training/unseen shapes per class.  Shown numbers are multiplied by $10^3$. The voxel oracle methods \{Vox-128,Vox-256,Vox-512\} measure the degradation alone due to voxelization (no learning).}
% \label{tab:chamfer}
% \end{table}
